Adaptive Out-Orientations with Applications

We give improved algorithms for maintaining edge-orientations of a fully-dynamic graph, such that the out-degree of each vertex is bounded. On one hand, we show how to orient the edges such that the out-degree of each vertex is proportional to the arboricity $\alpha$ of the graph, in, either, an amortised update time of $O(\log^2 n \log \alpha)$, or a worst-case update time of $O(\log^3 n \log \alpha)$. On the other hand, motivated by applications including dynamic maximal matching, we obtain a different trade-off, namely either $O(\log n \log \alpha)$, amortised, or $O(\log ^2 n \log \alpha)$, worst-case time, for the problem of maintaining an edge-orientation with at most $O(\alpha + \log n)$ out-edges per vertex. Since our algorithms have update times with worst-case guarantees, the number of changes to the solution (i.e. the recourse) is naturally limited. Our algorithms adapt to the current arboricity of the graph, and yield improvements over previous work: Firstly, we obtain an $O(\varepsilon^{-6}\log^3 n \log \rho)$ worst-case update time algorithm for maintaining a $(1+\varepsilon)$ approximation of the maximum subgraph density, $\rho$. Secondly, we obtain an $O(\varepsilon^{-6}\log^3 n \log \alpha)$ worst-case update time algorithm for maintaining a $(1 + \varepsilon) \cdot OPT + 2$ approximation of the optimal out-orientation of a graph with adaptive arboricity $\alpha$. This yields the first worst-case polylogarithmic dynamic algorithm for decomposing into $O(\alpha)$ forests.Thirdly, we obtain arboricity-adaptive fully-dynamic deterministic algorithms for a variety, of problems including maximal matching, $\Delta+1$ coloring, and matrix vector multiplication. All update times are worst-case $O(\alpha+\log^2n \log \alpha)$, where $\alpha$ is the current arboricity of the graph.

==> introtable.tex <==
\begin{table}[h]
\vspace{1em}
    \centering
    \begin{tabularx}{1.1\textwidth}{c|c|c|c|l}
      \makecell{\textbf{Dynamic} \\
     \textbf{Problem} 
     } & \textbf{Guarantee} & \makecell{\textbf{Worst-case Time}\\
     \textcolor{teal!80!black}{\textbf{Amortized Time}}} & \textbf{Thm.} & \textbf{State-of-the-art comparison} \\
         \hline
         \hline
     %
     %   CONSTANT FACTOR
     %
    \makecell{out-orient \\ /density}
     & 
     \makecell{  $\BigOh(\alpha)$ \\  $\BigOh(\rho)$}      & \makecell{$\BigOh( \log^3 n \log \alpha)$\\
     \textcolor{teal!80!black}{$\BigOh(\log^2 n)$}
     } & Thm.~\ref{thm:fastnonadd} & 
     \makecell[l]{
       $\BigOh(\alpha_{\mx}) \textnormal{ in } \BigOh(\alpha_{\mx} + \log n) \sim \textnormal{amor.~\cite{Brodal99dynamicrepresentations}}$ \\
      $\BigOh(\alpha) \textnormal{ in } \BigOh(\log^2 n) \sim \textnormal{amor.~\cite{henzinger2020explicit}}$ \\
      $\BigOh(\alpha) \textnormal{ in } \BigOh(\log^4 n) \sim \textnormal{implicit~\cite{sawlani2020near}}$
     }\\
     \hline
     % 
     % ADDITIVE LOG
     %
     \makecell{out-orient \\ /density} & 
      \makecell{  $\BigOh(\alpha + \log n)$ \\  $\BigOh(\rho + \log n)$} & 
      \makecell{$\BigOh(\log ^2 n \log \alpha)$\\
      \textcolor{teal!80!black}{$\BigOh(\log n)$}
      }& Thm.~\ref{thm:fast_butworse} &      
     \makecell[l]{
       $\BigOh(\alpha_{\mx} + \log n) \textnormal{ in } \BigOh(\log n)  \textnormal{~\cite{berglinetal:LIPIcs:2017:8263}}$ \\
      $\BigOh(\alpha + \log n) \textnormal{ in } \BigOh(  \alpha^2 + \log^2 n ) \textnormal{~\cite{KopelowitzKPS13}}$\\
      $\BigOh(\alpha) \textnormal{ in } \BigOh(\log^4 n) \sim \textnormal{implicit~\cite{sawlani2020near}}$
} \\
     \hline
     %
     % EPSILON DENSITY
     %
     density & $ (1 + \eps) \rho $ & \makecell{$\BigOh\paren*{\varepsilon^{-6}\log^3 n \log \rho}$\\
     \textcolor{teal!80!black}{$\BigOh\paren*{\varepsilon^{-4}\log^2 n}$}
     } & Cor.~\ref{cor:eps_subgraphdensity} & 
     \makecell[l]{
      $(1 + \eps) \rho \textnormal{ in } \BigOh(\eps^{-6} \log^4 n  ) \textnormal{~\cite{sawlani2020near}} $
     } \\
     \hline
    %
     % 2 EPSILON OUT 
     %
    out-orient & $(2 + \eps) \alpha + 1$ & \makecell{$\BigOh\paren*{\varepsilon^{-6}\log^3 n \log \alpha}$\\
    \textcolor{teal!80!black}{$\BigOh\paren*{\varepsilon^{-4}\log^2 n}$}
    } & Obs.~\ref{obs:rounding} & 
        $(2 + \eps) \alpha \textnormal{ in } \BigOh(\eps^{-6} \log^4 n  ) \sim \textnormal{implicit~\cite{sawlani2020near}}$
     \\
     %%%%%
     % 2 EPS OUT
     %%%%
     \hline
     out-orient & $(1 + \eps)\alpha + 2$ & $\BigOh( \eps^{-6} \log^3 n \log \alpha)$ & Thm.~\ref{thm:epsapprox} & 
     $
     \BigOh( \eps^{-6} \alpha^2 \log^3 n) \textnormal{~\cite{christiansenICALP}}
     $ \\
     %
     % MAX MATCHING
     %
     \hline
      \makecell{maximal \\ matching}  & -- & $\BigOh(\alpha + \log ^2 n \log \alpha)$ & Cor.~\ref{cor:match} & 
     \makecell[l]{$%
    \BigOh(\alpha_{\mx} + \log n) \textnormal{~ \cite{berglinetal:LIPIcs:2017:8263}}$ \\
       $\BigOh(\alpha_{\mx}+\sqrt{\alpha_{\mx}\log n} ) \sim\textnormal{amor.~\cite{HeTZ14}}$\\
       $\BigOh(\sqrt{m} )  \textnormal{~\cite{NeimanS16}}$ \\
     $\BigOh(\alpha^2 + \log^2 n) \textnormal{~\cite{KopelowitzKPS13}}%
     $} \\
     % 
     % DYNAMIC MATRIX MULTI
     %
       \hline
     \makecell{ maintain \\
     $A \cdot \overrightarrow{x}$} & -- & \makecell{$\BigOh(\log ^2 n \log \alpha)$ 
     for $A$ 
     \\
     $\BigOh(\alpha + \log n)$  \textnormal{ for }  $\overrightarrow{x}$ \\
     $\BigOh(\alpha + \log n)$  \textnormal{ query } 
     } & Cor.~\ref{cor:dynamicmatrix} &
  \makecell[l]{
     $\BigOh(\alpha^2 + \log^2 n) \textnormal{ updating } A$ \\
     $\BigOh(\alpha + \log n) \textnormal{ query+upd } \overrightarrow{x} 
     $
     \cite{KopelowitzKPS13}
    }
      \\
     %
     % FOREST DECOMP
     %
     \hline
     \makecell{ arboricity \\
     decomp } 
     & $\BigOh(\alpha)$ & $\BigOh(\log^3 n \log \alpha)$ & Cor.~\ref{cor:decomp} &
     \makecell[l]{
     $\BigOh(\alpha) \textnormal{ in } \BigOh(\log^2 n) \sim \textnormal{amor. }$
     \cite{henzinger2020explicit} \\ 
     $\BigOh(\sqrt{m}\log n)$ \cite{Banerjee}
     }
     \\
     \hline
    \makecell{ $\Delta+1$ \\
     coloring } 
     &  & $\BigOh(\alpha+\log^2 n\log \alpha)$ & Cor.~\ref{cor:col} &
     $\BigOh(\Delta)$ (folklore)
    \end{tabularx}
    \caption{
    Our results, compared to the state-of-the art. Unless mentioned otherwise, all algorithms are deterministic, have a worst case running times, and are fully-adaptive to the aboricity, and all orientations are stored explicitly.
    We denote by $\alpha$ the arboricity of the graph and by $\rho$ the maximal subgraph density. 
%    By using the notation $\widetilde{O}(f(n))$, we hide factors polynomial in $\log f(n)$.
    In the column comparing with state-of-the-art, we have indicated with ``$\sim$ implicit'' when the cited paper only gives implicit access to the solution it is maintaining, and we have indicated with ``$\sim$ amor.'' when the cited paper only gives an amortized running time. 
    \label{tab:results}
    }
\end{table}
